Federated Learning for Vision-based Obstacle Avoidance in the Internet of Robotic Things

Deep learning methods have revolutionized mobile robotics, from advanced perception models for an enhanced situational awareness to novel control approaches through reinforcement learning. This paper explores the potential of federated learning for distributed systems of mobile robots enabling collaboration on the Internet of Robotic Things. To demonstrate the effectiveness of such an approach, we deploy wheeled robots in different indoor environments. We analyze the performance of a federated learning approach and compare it to a traditional centralized training process with a priori aggregated data. We show the benefits of collaborative learning across heterogeneous environments and the potential for sim-to-real knowledge transfer. Our results demonstrate significant performance benefits of FL and sim-to-real transfer for vision-based navigation, in addition to the inherent privacy-preserving nature of FL by keeping computation at the edge. This is, to the best of our knowledge, the first work to leverage FL for vision-based navigation that also tests results in real-world settings.

==> algs/pos_gd.tex <==


\begin{algorithm}[t]
    %
    %
    %
    \footnotesize
	\caption{\footnotesize Ground truth extraction}
	\label{alg:tracking}
	\KwIn{\\
	    \begin{tabular}{ll}
	        3D lidar point cloud:             & $\mathcal{P}$ \\
	        Last known MAV state:              & $ \textbf{p}^{k-1}_{MAV}, {\dot{\textbf{p}}_{MAV}}^{k-1}$ \\[+0.4em]
	    \end{tabular}
	}
	\KwOut{\\
	    \begin{tabular}{ll}
	        MAV state:      & \{${\textbf{p}^{k}_{MAV}}, \:\dot{\textbf{p}}^{k}_{MAV}\}$ \\[+0.2em] 
	    \end{tabular}
	}  
	%\BlankLine
	%
	\SetKwFunction{FSub}{$object\_extraction\left(\mathcal{P}, \:{\textbf{p}^{k-1}_{MAV}}, \:\dot{\textbf{p}}^{k-1}_{MAV}\right)$}
    \SetKwProg{Fn}{Function}{:}{}
    % Position estimation based on current PointCloud and last position and speed
    \BlankLine
%     \Fn{\FSub}
%     {
%             \vspace{.3em}
            
%             \KwRet ${\textbf{p}^{k}_{MAV}};$
%     }
% 	\BlankLine
    %
% 	$Adaptive\;Integrate\;Rate: I_{rate}$ \\
    % Calculate with high frequency, get the pose(high accuracy, but not robust)  
    % Coarse first, then fine grained estimate
    % \tcp{Coarse but persistent tracking}
    % \While{new $\mathcal{P}_{k}(I^{k}_{MF})$}{
    %     ${\textbf{p}^{k'}_{MAV}} =  object\_extraction(\mathcal{P}_{k}(I^{k}_{MF}), I^{k}_{MF}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
    %     % $Evaluate \; Estimation({\textbf{p}^{k-1}_{MAV}}, {\textbf{p}^{k}_{MAV}} )$ \\
    %     % $Update({\textbf{p}}^{k}, I_{rate} )$ \\
    % }
    % \tcp{Fine-grained estimation}
    \While{new $\mathcal{P}_{k}$}{
        \begin{tabular}{ll}
                Generate KD Tree:       & $kdtree \leftarrow \mathcal{P};$ \\
                MAV pos estimation:     & $\hat{\textbf{p}}_{\tiny MAV}^{k} \leftarrow \textbf{p}^{k-1}_{MAV} + \frac{\dot{\textbf{p}}_{MAV}^{k-1}}{I};$ \\[+0.4em]
                MAV points:             & $\mathcal{P}^{k}_{MAV} = KNN(kdtree, \: \hat{\textbf{p}}_{MAV}^{k});$ \\[+0.4em]
                MAV state estimation:   & ${\textbf{p}^{k}_{MAV}} = \frac{1}{\lvert\mathcal{P}^{k}_{MAV}\rvert}\sum_{p\in\mathcal{P}^{k}_{MAV}} p;$ \\
        \end{tabular}
        % ${\textbf{p}^{k''}_{MAV}} =  object\_extraction(\mathcal{P}_{k}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
        % ${\textbf{p}^{k}_{MAV}}, \: {\dot{\textbf{p}}^{k}_{MAV}} \leftarrow estimate\left(\textbf{p}^{k'}_{MAV}, \:\textbf{p}^{k''}_{MAV}\right)$\;
    }
    % $\{I^{k}_{HF}, I^{k}_{MF}\} \leftarrow adjust\_integration\_freqs\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$ \\[+0.4em]
    % $\dot{\textbf{q}}^{k}_{UGV} \leftarrow keep\_within\_FoV\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$
    
 
\end{algorithm}

==> tex/data_combinations.tex <==
\begin{table}[t]
    \caption{\footnotesize The Training Data Combinations and Their Acronyms}
    \scriptsize
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        \textbf{Combinations} & \textbf{TD0\&TD1} & \textbf{TD0\&TD2} & \textbf{TD1\&TD2} & \textbf{TD0\&TD1\&TD2} \\
        \midrule
        \textbf{Acronyms}     & TD01                & TD02                & TD12                & TD012                      \\
        \bottomrule
    \end{tabular}
    \label{tab:data_combination}
\end{table}

==> tex/fuse_combinations.tex <==
\begin{table}[t]
    \centering
    \caption{\footnotesize Fused Model Combination Acronyms}
    \label{tab:fuse_combination}
    \scriptsize
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        \textbf{Combinations} & \textbf{M0\&M1} & \textbf{M0\&M2} & \textbf{M1\&M2} & \textbf{M0\&M1\&M2} \\ 
        \midrule
        \textbf{Acronyms}     & M01                & M02                & M12                & M012                      \\ 
        \bottomrule
    \end{tabular}
\end{table}
